The Persian Dependency Treebank Made Universal

We describe an automatic method for converting the Persian Dependency Treebank (Rasooli et al, 2013) to Universal Dependencies. This treebank contains 29107 sentences. Our experiments along with manual linguistic analysis show that our data is more compatible with Universal Dependencies than the Uppsala Persian Universal Dependency Treebank (Seraji et al., 2016), and is larger in size and more diverse in vocabulary. Our data brings in a labeled attachment F-score of 85.2 in supervised parsing. Our delexicalized Persian-to-English parser transfer experiments show that a parsing model trained on our data is ~2% absolutely more accurate than that of Seraji et al. (2016) in terms of labeled attachment score.

==> analysis.tex <==
Points to be considered:
%1. Seraji has mistakenly not determined csubj label in her analysis of Persian syntax. In a sentence like "لازم است او بیاید" (it is necessary for him to come), it is obvious that what comes after "است", is the clausal subject of the adjectival sentence predicate which is "لازم". A simple syntactic test supports the viewpoint. One can convert the clausal complement "او بیاید" to a noun phrase "آمدن او" and reanalyze the sentence. In this case, the phrase "آمدن او" which is the converted version of the clausal complement, plays the nsubj role of the sentence. Therefore, the clausal complement of the sentence is specified as csubj.
2. Seraji has incorrectly considered prepositional and possessive complements of adjectival heads as nmod (sentid = train-s2490) and nmod:poss (sentid = train-s4481) respectively. Her analysis clearly stands in contradiction to UD annotation guideline in which nmod label is used just for dependents of a nominal head not an adjectival one. What UD and also PUD corpus suggests for the mentioned dependents is obl.
%3. As another clear contradiction to UD guideline, one can consider her analysis of "شدن" (to become) as cop (sentid = train-s30, sentid = train-s3787). What UD asserts under the cop label is that "…the equivalents of to become are not copulas despite the fact that traditional grammar may label them as such." In other words, شدن should have been deemed as a verbal predicate and its second complement as xcomp. 
%4. As Moloodi and Kouhestani (2017) states, Persian has a frequent two-word light verb which is "پیدا کردن". Its combination with non-verbal elements yields complex predicates like "ادامه پیدا کردن، غلبه پیدا کردن، انجام پیدا کردن". Following Moloodi and Kouhestani (2017), in the present research, the word "پیدا" is considered as one part of the two-word light verb and the compound:lv label is assigned to it. Based on UD guideline, the nonverbal elements of these complex predicates are annotated as compound:lvc, as well. However, Seraji has incorrectly annotated the nonverbal elements of these complex predicates as obj and considers "پیدا" as a nonverbal element not as a part of a two-word light verb.
5. Another syntactic label which is absent in Seraji's is iobj. Its absence may be due to the low frequency of this syntactic relation in Persian. Anyway, in Dadegan Universal Dependencies (DUDE), there are 7 cases of this relation.
 


==> figures/vconj_map.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[]{trees/vconj/vconj}
	\caption{Our rotation rule for changing the order of verbal conjunctions (VCONJ). Note that $c_x$s are usually coordinating conjunctions (mostly the word \setfarsi\novocalize \<w>).} 
	\label{fig:vconj_rotation}
\end{figure}

==> label_freq.tex <==
\begin{comment}
\begin{table*}[t!]
	\small
	\centering
	\begin{tabular}{|l|c|c |l|c|c |l|c|c |}
		\hline
		Label  & \#    & \%    & Label   & \#    & \%    & Label & \#    & \%     \\ \hline
		case        & 70206 & 13.7  & conj         & 23616 & 4.6   & acl        & 10035 & 1.9    \\ \hline
		obl         & 28249 & 5.5   & punct        & 44306 & 8.7   & cop        & 6364  & 1.2    \\ \hline
		det         & 10193 & 2     & advmod       & 13383 & 2.6   & aux:pass   & 822   & 0.1    \\ \hline
		nmod        & 59442 & 11.6  & appos        & 1059  & 0.2   & aux        & 12886 & 0.16   \\ \hline
		amod        & 22593 & 4.4   & compound:lvc & 32339 & 6.3   & nsubj:pass & 530   & 0.1    \\ \hline
		nsubj       & 27355 & 5.3   & name:flat    & 7895  & 1.5   & dep        & 2033  & 0.3    \\ \hline
		cc          & 21083 & 4.1   & root         & 29107 & 5.7   & advcl      & 4231  & 0.8    \\ \hline
		obj         & 19999 & 3.9   & xcomp        & 4920  & 0.9   & parataxis  & 82    & 0.01   \\ \hline
		ccomp       & 6940  & 1.3   & obl:arg      & 21302 & 4.1   & flat:num   & 588   & 0.1    \\ \hline
		nummod      & 5420  & 1     & mark         & 11986 & 2.3   & fixed      & 1468  & 0.2    \\ \hline
		compound:lv & 439   & 0.08  & csubj        & 682   & 0.1   & vocative   & 174   & 0.03   \\ \hline
		compound    & 42    & 0.008 & iobj         & 6     & 0.001 & dislocated & 1     & 0.0001 \\ \hline
	\end{tabular}
	
	\caption{Frequency of each universal label  the converted dataset.}\label{tab:univ_freq}
\end{table*}
\end{comment}

\begin{figure*}
	

\pgfplotstableread[row sep=\\,col sep=&]{
	label & frequency & percentage \\
case & 70206 & 13.7 \\ 
nmod & 59442 & 11.6 \\ 
punct & 44306 & 8.7 \\ 
compound:lvc & 32339 & 6.3 \\ 
root & 29107 & 5.7 \\ 
obl & 28249 & 5.5 \\ 
nsubj & 27355 & 5.3 \\ 
conj & 23616 & 4.6 \\ 
amod & 22593 & 4.4 \\ 
obl:arg & 21302 & 4.1 \\ 
cc & 21083 & 4.1 \\ 
obj & 19999 & 3.9 \\ 
advmod & 13383 & 2.6 \\ 
 aux & 12886 & 0.16 \\ 
 mark & 11986 & 2.3 \\ 
det & 10193 & 2 \\ 
acl & 10035 & 1.9 \\ 
name:flat & 7895 & 1.5 \\ 
ccomp & 6940 & 1.3 \\ 
cop & 6364 & 1.2 \\ 
nummod & 5420 & 1 \\ 
xcomp & 4920 & 0.9 \\ 
advcl & 4231 & 0.8 \\ 
dep & 2033 & 0.3 \\ 
fixed & 1468 & 0.2 \\ 
appos & 1059 & 0.2 \\
aux:pass & 822 & 0.1 \\ 
csubj & 682 & 0.1 \\ 
flat:num & 588 & 0.1 \\ 
nsubj:pass & 530 & 0.1 \\ 
compound:lv & 439 & 0.08 \\ 
vocative & 174 & 0.03 \\ 
parataxis & 82 & 0.01 \\ 
compound & 42 & 0.008 \\ 
iobj & 6 & 0.001 \\ 
dislocated & 1 & 0.0001 \\
goeswith & 1 & 0.0001 \\
}\mydata

\centering
\scalebox{0.2}{
\begin{tikzpicture}
\begin{axis}[
ybar,
ymin=1,
ymode=log,
symbolic x  coords={case,nmod,punct,compound:lvc,root,obl,nsubj,conj,amod,obl:arg,cc,obj,advmod,aux,mark,det,acl,name:flat,ccomp,cop,nummod,xcomp,advcl,dep,fixed,appos,aux:pass,csubj,flat:num,nsubj:pass,compound:lv,vocative,parataxis,compound,iobj,dislocated,goeswith},
  every node near coord/.append style={font=\tiny},
xtick=data,
    width  = 4*\textwidth,
]
\addplot table[x=label,y=frequency]{\mydata};
\end{axis}
\end{tikzpicture}
}
	\caption{Percentage of each universal label  the converted dataset.}\label{tab:univ_freq}
\end{figure*}


==> tables/delex_results.tex <==
\begin{table}[t!]
	\centering
		\begin{tabular}{l c c}
	Data & UAS & LAS \\ \hline
	UDT & 45.37 & 36.42 \\
	PerDT & {\bf 47.31} & {\bf 38.59} \\
\end{tabular}
\end{table}

==> tables/experiment_tables.tex <==
seraji Seraji test.conllu
Metric     | Precision |    Recall |  F1 Score | AligndAcc
-----------+-----------+-----------+-----------+-----------
Tokens     |    100.00 |    100.00 |    100.00 |
Sentences  |    100.00 |    100.00 |    100.00 |
Words      |     99.68 |     99.50 |     99.59 |
UPOS       |     95.84 |     95.66 |     95.75 |     96.14
XPOS       |      0.00 |      0.00 |      0.00 |      0.00
UFeats     |     99.68 |     99.50 |     99.59 |    100.00
AllTags    |      0.00 |      0.00 |      0.00 |      0.00
Lemmas     |     89.63 |     89.47 |     89.55 |     89.92
UAS        |     83.58 |     83.43 |     83.51 |     83.85
LAS        |     79.49 |     79.34 |     79.42 |     79.74
CLAS       |     74.88 |     74.68 |     74.78 |     75.15
MLAS       |     73.11 |     72.92 |     73.01 |     73.37
BLEX       |     65.62 |     65.45 |     65.53 |     65.85

 seraji Dadegan test.conllu
Metric     | Precision |    Recall |  F1 Score | AligndAcc
-----------+-----------+-----------+-----------+-----------
Tokens     |     99.94 |     99.93 |     99.93 |
Sentences  |    100.00 |    100.00 |    100.00 |
Words      |     98.82 |     98.63 |     98.73 |
UPOS       |     81.74 |     81.58 |     81.66 |     82.71
XPOS       |      0.00 |      0.00 |      0.00 |      0.00
UFeats     |     98.82 |     98.63 |     98.73 |    100.00
AllTags    |      0.00 |      0.00 |      0.00 |      0.00
Lemmas     |     79.84 |     79.68 |     79.76 |     80.79
UAS        |     70.81 |     70.67 |     70.74 |     71.66
LAS        |     64.01 |     63.88 |     63.95 |     64.77
CLAS       |     60.17 |     58.56 |     59.35 |     59.71
MLAS       |     49.70 |     48.38 |     49.03 |     49.32
BLEX       |     44.81 |     43.62 |     44.20 |     44.47

Dadegan->Dadegan
Metric     | Precision |    Recall |  F1 Score | AligndAcc
-----------+-----------+-----------+-----------+-----------
Tokens     |     99.99 |     99.99 |     99.99 |
Sentences  |    100.00 |    100.00 |    100.00 |
Words      |     99.71 |     99.56 |     99.63 |
UPOS       |     96.23 |     96.08 |     96.16 |     96.51
XPOS       |     96.05 |     95.91 |     95.98 |     96.33
UFeats     |     99.71 |     99.56 |     99.63 |    100.00
AllTags    |     95.01 |     94.86 |     94.94 |     95.29
Lemmas     |     96.32 |     96.18 |     96.25 |     96.60
UAS        |     88.64 |     88.50 |     88.57 |     88.90
LAS        |     85.51 |     85.38 |     85.45 |     85.76
CLAS       |     82.08 |     81.67 |     81.88 |     82.18
MLAS       |     79.45 |     79.05 |     79.25 |     79.54
BLEX       |     78.69 |     78.29 |     78.49 |     78.78

dadegan Seraji test.conllu
Metric     | Precision |    Recall |  F1 Score | AligndAcc
-----------+-----------+-----------+-----------+-----------
Tokens     |    100.00 |    100.00 |    100.00 |
Sentences  |    100.00 |    100.00 |    100.00 |
Words      |     99.68 |     99.49 |     99.58 |
UPOS       |     81.92 |     81.76 |     81.84 |     82.19
XPOS       |      0.00 |      0.00 |      0.00 |      0.00
UFeats     |     99.68 |     99.49 |     99.58 |    100.00
AllTags    |      0.00 |      0.00 |      0.00 |      0.00
Lemmas     |     90.48 |     90.30 |     90.39 |     90.77
UAS        |     69.81 |     69.67 |     69.74 |     70.03
LAS        |     62.49 |     62.37 |     62.43 |     62.69
CLAS       |     56.60 |     57.90 |     57.24 |     58.26
MLAS       |     45.75 |     46.80 |     46.27 |     47.09
BLEX       |     52.02 |     53.22 |     52.61 |     53.55

